Term Ordering Diagrams

The superposition calculus for reasoning in first-order logic with equality relies on simplification orderings on terms. Modern saturation provers use the Knuth-Bendix order (KBO) and the lexicographic path order (LPO) for discovering redundant clauses and inferences. Implementing term orderings is however challenging. While KBO comparisons can be performed in linear time and LPO checks in quadratic time, using the best known algorithms for these orders is not enough. Indeed, our experiments show that for some examples term ordering checks may use about 98% of the overall proving time. The reason for this is that some equalities that cannot be ordered can become ordered after applying a substitution (post-ordered), and we have to check for post-ordering repeatedly for the same equalities. In this paper, we show how to improve post-ordering checks by introducing a new data structure called term ordering diagrams, in short TODs, which creates an index for these checks. We achieve efficiency by lazy modifications of the index and by storing and reusing information from previously performed checks to speed up subsequent checks. Our experiments demonstrate efficiency of TODs.

==> misc.tex <==

\section*{Longer example}

\begin{example}

Given the ordering diagram from our motivating example and $\theta=\emptyset$, i.e. a renaming, we get the following transformations.

\begin{center}
\begin{tikzpicture}
\node[] (source) at (-1,0) {};
\node[termnode=above:1.1,processed] (c11) at (0,0) {$x\comp y$};
\node[termnode=above:1.2] (c12) at (3,0) {$f(y,z)\comp f(z,x)$};
\node[termnode=above:2] (c2) at (6,0) {$s\comp u$};
\node[datanode=below:3] (s1) at (0,-2) {$s\eqs t$};
\node[datanode=below:4] (s2) at (3,-2) {$s\eqs u$};
\node[sinknode] (fail) at (6,-2) {};

\altbranch{source}{c11};

\gtbranch[]{c11}{s1};
\eqbranch[]{c11}{c12};
\incbranch[bend left=30]{c11}{c2};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c2};
\incbranch[bend left=20]{c12}{c2};

\gtbranch[]{c2}{s2};
\eqbranch[bend right]{c2}{fail};
\incbranch[bend left]{c2}{fail};

\altbranch[]{s1}{c2};
\altbranch[]{s2}{fail};

\end{tikzpicture}
\end{center}

\begin{center}
\begin{tikzpicture}
\node[] (source) at (-1,0) {};
\node[termnode=above:1.1,processed] (c11) at (0,0) {$x\comp y$};
\node[termnode=above:1.2] (c12) at (3,0) {$f(y,z)\comp f(z,x)$};
\node[termnode=above:2.1] (c21) at (6,0) {$x\comp z$};
\node[termnode=above:2.2] (c22) at (9,0) {$f(y,z)\comp f(x,y)$};
\node[datanode=below:3] (s1) at (1.5,-2) {$s\eqs t$};
\node[datanode=below:4] (s2) at (4.5,-2) {$s\eqs u$};
\node[sinknode] (fail) at (7.5,-2) {};

\altbranch{source}{c11};

\gtbranch[]{c11}{s1};
\eqbranch[]{c11}{c12};
\incbranch[bend left=30]{c11}{c21};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c21};
\incbranch[bend left=20]{c12}{c21};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};
\incbranch[]{c21}{fail};

\gtbranch[]{c22}{s2};
\eqbranch[bend left]{c22}{fail};
\incbranch[bend right=10]{c22}{fail};

\altbranch[]{s1}{c21};
\altbranch[]{s2}{fail};

\end{tikzpicture}
\end{center}


\begin{center}
\begin{tikzpicture}
\node[] (source) at (-1,0) {};
\node[termnode=above:1.1,processed] (c11) at (0,0) {$x\comp y$};
\node[termnode=above:1.2] (c12) at (3,0) {$f(y,z)\comp f(z,x)$};
\node[termnode=above:2.1,processed] (c21) at (6,.7) {$x\comp z$};
\node[termnode=above:2.1'] (c21') at (6,-.7) {$x\comp z$};
\node[termnode=above:2.2] (c22) at (9,0) {$f(y,z)\comp f(x,y)$};
\node[datanode=below:3] (s1) at (1.5,-2) {$s\eqs t$};
\node[datanode=below:4] (s2) at (4.5,-2) {$s\eqs u$};
\node[sinknode] (fail) at (7.5,-2) {};

\altbranch{source}{c11};

\gtbranch[]{c11}{s1};
\eqbranch[]{c11}{c12};
\incbranch[bend left=15]{c11}{c21};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c21'};
\incbranch[bend left=20]{c12}{c21'};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};
\incbranch[]{c21}{fail};

\gtbranch[]{c21'}{s2};
\eqbranch[]{c21'}{c22};
\incbranch[]{c21'}{fail};

\gtbranch[]{c22}{s2};
\eqbranch[bend left]{c22}{fail};
\incbranch[bend right=10]{c22}{fail};

\altbranch[]{s1}{c21'};
\altbranch[]{s2}{fail};

\end{tikzpicture}
\end{center}

Let us ``execute'' the diagram again, with $\theta'=\{x\mapsto y\}$.

\begin{center}
\begin{tikzpicture}
\node[] (source) at (-1,0) {};
\node[termnode=above:1.1,processed] (c11) at (0,0) {$x\comp y$};
\node[termnode=below right:1.2.1,processed] (c121) at (2,0) {$y\comp z$};
\node[termnode=below:1.2.2] (c122) at (4,-.2) {$z\comp x$};
\node[termnode=above:2.1,processed] (c21) at (6,.7) {$x\comp z$};
\node[termnode=above:2.1'] (c21') at (6,-.7) {$x\comp z$};
\node[termnode=above:2.2] (c22) at (9,0) {$f(y,z)\comp f(x,y)$};
\node[datanode=below:3] (s1) at (1.5,-2) {$s\eqs t$};
\node[datanode=below:4] (s2) at (4.5,-2) {$s\eqs u$};
\node[sinknode] (fail) at (7.5,-2) {};

\altbranch{source}{c11};

\gtbranch[]{c11}{s1};
\eqbranch[]{c11}{c121};
\incbranch[bend left=15]{c11}{c21};

\gtbranch[]{c121}{s1};
\eqbranch[]{c121}{c122};
\incbranch[bend left]{c121}{c21'};

\gtbranch[]{c122}{s1};
\eqbranch[bend right=20]{c122}{c21'};
\incbranch[bend left=20]{c122}{c21'};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};
\incbranch[]{c21}{fail};

\gtbranch[]{c21'}{s2};
\eqbranch[]{c21'}{c22};
\incbranch[]{c21'}{fail};

\gtbranch[]{c22}{s2};
\eqbranch[bend left]{c22}{fail};
\incbranch[bend right=10]{c22}{fail};

\altbranch[]{s1}{c21'};
\altbranch[]{s2}{fail};

\end{tikzpicture}
\end{center}
At this point, we look reach a node with $x\succ z$, but since we have gone through $x=y$ and $y\succ z$, this is already true on this branch.
\begin{center}
\begin{tikzpicture}
\node[] (source) at (-1,0) {};
\node[termnode=above:1.1,processed] (c11) at (0,0) {$x\comp y$};
\node[termnode=above right:1.2.1,processed] (c121) at (2,0) {$y\comp z$};
\node[termnode=above:1.2.2] (c122) at (4,-.2) {$z\comp x$};
\node[termnode=above:2.1,processed] (c21) at (6,.7) {$x\comp z$};
\node[termnode=above:2.1'] (c21') at (6,-.7) {$x\comp z$};
\node[termnode=above:2.2] (c22) at (9,0) {$f(y,z)\comp f(x,y)$};
\node[datanode=below:3] (s1) at (1.5,-2) {$s\eqs t$};
\node[datanode=below:4] (s2) at (4.5,-2) {$s\eqs u$};
\node[sinknode] (fail) at (7.5,-2) {};

\altbranch{source}{c11};

\gtbranch[]{c11}{s1};
\eqbranch[]{c11}{c121};
\incbranch[bend left=15]{c11}{c21};

\gtbranch[]{c121}{s1};
\eqbranch[]{c121}{c122};
\incbranch[]{c121}{s2};

\gtbranch[]{c122}{s1};
\eqbranch[bend right=20]{c122}{c21'};
\incbranch[bend left=20]{c122}{c21'};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};
\incbranch[]{c21}{fail};

\gtbranch[]{c21'}{s2};
\eqbranch[]{c21'}{c22};
\incbranch[]{c21'}{fail};

\gtbranch[]{c22}{s2};
\eqbranch[bend left]{c22}{fail};
\incbranch[bend right=10]{c22}{fail};

\altbranch[]{s1}{c21'};
\altbranch[]{s2}{fail};

\end{tikzpicture}
\end{center}
We get the $s\eqs u$. Let us execute again with $\theta''=\{x\mapsto y, z\mapsto y\}$.
\begin{center}
\begin{tikzpicture}
\node[] (source) at (-1,0) {};
\node[termnode=above:1.1,processed] (c11) at (0,0) {$x\comp y$};
\node[termnode=above right:1.2.1,processed] (c121) at (3,0) {$y\comp z$};
\node[termnode=above:2.1,processed] (c21) at (6,.7) {$x\comp z$};
\node[termnode=above:2.1'] (c21') at (6,-.7) {$x\comp z$};
\node[termnode=above:2.2.1] (c221) at (8,0) {$y\comp x$};
\node[termnode=above:2.2.2] (c222) at (10,0) {$z\comp y$};
\node[datanode=below:3] (s1) at (1.5,-2) {$s\eqs t$};
\node[datanode=below:4] (s2) at (4.5,-2) {$s\eqs u$};
\node[sinknode] (fail) at (7.5,-2) {};

\altbranch{source}{c11};

\gtbranch[]{c11}{s1};
\eqbranch[]{c11}{c121};
\incbranch[bend left=10]{c11}{c21};

\gtbranch[]{c121}{s1};
\eqbranch[]{c121}{c221};
\incbranch[]{c121}{s2};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c221};
\incbranch[]{c21}{fail};

\gtbranch[]{c21'}{s2};
\eqbranch[]{c21'}{c221};
\incbranch[]{c21'}{fail};

\gtbranch[]{c221}{s2};
\eqbranch[bend left]{c221}{c222};
\incbranch[bend right=10]{c221}{c222};

\gtbranch[]{c222}{s2};
\eqbranch[bend left=15]{c222}{fail};
\incbranch[bend right=10]{c222}{fail};

\altbranch[]{s1}{c21'};
\altbranch[]{s2}{fail};

\end{tikzpicture}
\end{center}
Since we have $x=y$ and $y=z$ on this path, we can infer $y=x$ and $z=y$, hence we can point to the fail node in two steps.
\begin{center}
\begin{tikzpicture}
\node[] (source) at (-1,0) {};
\node[termnode=above:1.1,processed] (c11) at (0,0) {$x\comp y$};
\node[termnode=above right:1.2.1,processed] (c121) at (3,0) {$y\comp z$};
\node[termnode=above:2.1,processed] (c21) at (6,.7) {$x\comp z$};
\node[termnode=above:2.1'] (c21') at (6,-.7) {$x\comp z$};
\node[termnode=above:2.2.1] (c221) at (8,0) {$y\comp x$};
\node[termnode=above:2.2.2] (c222) at (10,0) {$z\comp y$};
\node[datanode=below:3] (s1) at (1.5,-2) {$s\eqs t$};
\node[datanode=below:4] (s2) at (4.5,-2) {$s\eqs u$};
\node[sinknode] (fail) at (7.5,-2) {};

\altbranch{source}{c11};

\gtbranch[]{c11}{s1};
\eqbranch[]{c11}{c121};
\incbranch[bend left=10]{c11}{c21};

\gtbranch[]{c121}{s1};
\eqbranch[bend right=10]{c121}{fail};
\incbranch[]{c121}{s2};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c221};
\incbranch[]{c21}{fail};

\gtbranch[]{c21'}{s2};
\eqbranch[]{c21'}{c221};
\incbranch[]{c21'}{fail};

\gtbranch[]{c221}{s2};
\eqbranch[bend left]{c221}{c222};
\incbranch[bend right=10]{c221}{c222};

\gtbranch[]{c222}{s2};
\eqbranch[bend left=15]{c222}{fail};
\incbranch[bend right=10]{c222}{fail};

\altbranch[]{s1}{c21'};
\altbranch[]{s2}{fail};

\end{tikzpicture}
\end{center}
Try again with a substitution $\theta'''$ s.t. $x\theta'''\succ y\theta'''=z\theta'''$.
\begin{center}
\begin{tikzpicture}
\node[] (source) at (-1,0) {};
\node[termnode=above:1.1,processed] (c11) at (0,0) {$x\comp y$};
\node[termnode=above right:1.2.1,processed] (c121) at (3,0) {$y\comp z$};
\node[termnode=above:2.1,processed] (c21) at (6,.7) {$x\comp z$};
\node[termnode=above:2.1'] (c21') at (6,-.7) {$x\comp z$};
\node[termnode=above:2.2.1] (c221) at (8,0) {$y\comp x$};
\node[termnode=above:2.2.2] (c222) at (10,0) {$z\comp y$};
\node[datanode=below:3,processed] (s11) at (.5,-2) {$s\eqs t$};
\node[datanode=below:3'] (s12) at (2.5,-2) {$s\eqs t$};
\node[datanode=below:4] (s2) at (4.5,-2) {$s\eqs u$};
\node[sinknode] (fail) at (7.5,-2) {};

\altbranch{source}{c11};

\gtbranch[]{c11}{s11};
\eqbranch[]{c11}{c121};
\incbranch[bend left=10]{c11}{c21};

\gtbranch[]{c121}{s12};
\eqbranch[bend right=10]{c121}{fail};
\incbranch[]{c121}{s2};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c221};
\incbranch[]{c21}{fail};

\gtbranch[]{c21'}{s2};
\eqbranch[]{c21'}{c221};
\incbranch[]{c21'}{fail};

\gtbranch[]{c221}{s2};
\eqbranch[bend left]{c221}{c222};
\incbranch[bend right=10]{c221}{c222};

\gtbranch[]{c222}{s2};
\eqbranch[bend left=15]{c222}{fail};
\incbranch[bend right=10]{c222}{fail};

\altbranch[bend left=10]{s11}{c21'};
\altbranch[]{s12}{c21'};
\altbranch[]{s2}{fail};

\end{tikzpicture}
\end{center}
\end{example}

\section*{Unused stuff}

In this paper, we deal with the efficient implementation of term ordering checks with the following assumptions:
\begin{itemize}
\item The check is performed between terms $s\sigma$ and $t\sigma$ where $s$ and $t$ are arbitrary but \textit{fixed} terms and $\sigma$ is an arbitrary substitution.
\item The check is \textit{unidirectional} (as opposed to \textit{bidirectional}), i.e. we are only interested in distinguishing between $s\theta\succ t\theta$, $s\theta=t\theta$ and $s\theta\not\succeq t\theta$. In other words, we do not care whether $s\theta\prec t\theta$.
\end{itemize}
These assumptions cover a large number of practical situations. For example, we use an equation $s\eqs t$ to demodulate (or superpose) into different clauses under some substitution (resp. unifier) $\sigma$ potentially many times, hence we can assume that $s$ and $t$ are fixed. This allows further optimizations using \textit{runtime algorithm specialization}, as described later. Second, unidirectional checks are often enough in practice, and allow more optimizations (and a cleaner presentation).

Some notes on the problem we are facing:
\begin{itemize}
\item Usually, exploring non-failing paths in the ordering diagram worth the effort, as we get a simplification or redundant inference in exchange. However, failing paths need to be explored but are usually a waste of time. In any case, we only explore (and expand) parts of an ordering diagram as lazily as possible, to avoid exploring parts which will not be used at all, and there are usually many such paths.
\item Using unidirectional comparison (i.e. only differentiating between $l\succ r$ and $l\not\succ r$) is much less effort as using full bidirectional comparison (i.e. knowing exactly $l=r$, $l\prec r$ or $l\bowtie r$ in the $l\not\succ r$ case), but this gives us less information to skip later comparisons on a path. We hypothesize that the information we get from bidirectional comparisons is not worth it.
\item For both KBO and LPO, we also need to differentiate $l\succ r$, $l=r$ and $l\not\succeq r$. For example, the lexicographic comparisons require to be an "equal" branch. But LPO uses even more branching, see code below.
\end{itemize}

% \begin{minipage}{.5\linewidth}
% \begin{algorithmic}
% \Struct{\Node}
%     \State $\lbl$ : $\Label$
% \EndStruct
% \State
% \Struct{\FailNode{} : \Node}
%     \State $\lbl=\SINK$
% \EndStruct
% \State
% \Struct{\SuccessNode{} : \Node}
%     \State $\lbl=\DATA$
%     \State $\data$ : $D$
%     \State $\true$ : $\Branch$
% \EndStruct
% \end{algorithmic}
% \end{minipage}\begin{minipage}{.5\linewidth}
% \begin{algorithmic}
% \Struct{\WeightNode{} : \Node}
%     \State $\lbl=\POLY$
%     \State $\poly$ : $\Poly$
%     \State $\gt$ : $\Branch$
%     \State $\eq$ : $\Branch$
%     \State $\nge$ : $\Branch$
% \EndStruct
% \State
% \Struct{\ComparisonNode{} : \Node}
%     \State $\lbl=\COMP$
%     \State $\lhs$ : $\Terms$
%     \State $\rhs$ : $\Terms$
%     \State $\gt$ : $\Branch$
%     \State $\eq$ : $\Branch$
%     \State $\nge$ : $\Branch$
% \EndStruct
% \end{algorithmic}
% \end{minipage}

% Let $\Omega=(V,E,r,f)$ be an ordering diagram and $\theta$ a substitution. Let $P=v_0\to v_1\to \ldots\to v_n\to v$ be a satisfied path in $\Omega$ w.r.t. $\theta$ s.t. $v_0,v_1,\ldots,v_n$ are processed and $v$ is unprocessed.
% \begin{enumerate}[label=(\arabic*)]
% \item If $v=r$, $k(r)=\POLY$ or $k(r)=\COMP$, and $\exists (r,w)\in E.\models\constraint((r,w))$, then:
% %
% $$(V'\uplus\{r\},E,r,f)\Longrightarrow (V',E,w,f)$$
% \item If $k(v)=\POLY$ or $k(v)=\COMP$, and $\exists (v,w)\in E.\constraint(P)\models\constraint((v,w))$, then:
% %
% $$(V'\uplus\{v\},E'\uplus\{(v_n,v)\},r,f)\Longrightarrow (V',E'\cup \{(v_n,w)\},r,f)$$
% where $l((v_n,w))=l((v_n,v))$.
% \item If $k(v)\neq\COMP$ or $\lhs(v)\in\Vars$ or $\rhs(v)\in\Vars$, then:
% %
% $$(V,E'\uplus\{(v_n,v)\},r,f)\Longrightarrow (V\uplus\{v'\},E\cup \{(v_n,v')\},r,f)$$
% where $k(v')=k(v)$ and $l((v_n,v'))=l((v_n,v))$.
% \end{enumerate}


% \begin{minipage}{.5\linewidth}
% \begin{tikzpicture}[inner sep=2pt,subdag/.style = { regular polygon, regular polygon sides=3 }]
% \node (x) at (0,0) {$\ldots$};
% \node[termnode,processed] (y) at (3,0) {$M$};
% \node[termnode] (z) at (1.5,-1) {$N$};
% \node[subdag,draw=black] (gt) at (0,-3) {$T_1$};
% \node[subdag,draw=black] (eq) at (1.5,-3) {$T_2$};
% \node[subdag,draw=black] (inc) at (3,-3) {$T_3$};
% \path[->] (x.south west) edge[bend right] (z);
% \path[->] (x.south) edge[bend right] (z);
% \path[->] (x.south east) edge[bend right] (z);
% \draw[->] (y) -- (z);

% \branches{z}{gt.north}{eq.north}{inc.north}
% \end{tikzpicture}
% \end{minipage}\begin{minipage}{.5\linewidth}
% \begin{tikzpicture}[inner sep=2pt,subdag/.style = { regular polygon, regular polygon sides=3 }]
% \node (x) at (0,0) {$\ldots$};
% \node[termnode,processed] (y) at (3,0) {$M$};
% \node[termnode] (z) at (.5,-1) {$N$};
% \node[termnode,processed] (z') at (2.5,-1) {$N'$};
% \node[subdag,draw=black] (gt) at (0,-3) {$T_1$};
% \node[subdag,draw=black] (eq) at (1.5,-3) {$T_2$};
% \node[subdag,draw=black] (inc) at (3,-3) {$T_3$};
% \path[->] (x.south west) edge[bend right] (z);
% \path[->] (x.south) edge[bend right] (z);
% \path[->] (x.south east) edge[bend right] (z);
% \draw[->] (y) -- (z');

% \branches{z}{gt.north}{eq.north}{inc.north}
% \branches{z'}{gt.north}{eq.north}{inc.north}
% \end{tikzpicture}
% \end{minipage}

% If $s=f(s_1,...,s_n)$, $t=g(t_1,...,t_m)$ and $g\gg f$ and $p=|s|-|t|$.

% \begin{minipage}{.5\linewidth}
% \begin{tikzpicture}[inner sep=2pt,subdag/.style = { regular polygon, regular polygon sides=3 }]
% % \node[termnode,processed] (y) at (3,0) {$M$};
% \node[termnode] (z) at (1.5,-1) {$s\comp t$};
% \node[subdag,draw=black] (gt) at (0,-3) {$T_1$};
% \node[subdag,draw=black] (eq) at (1.5,-3) {$T_2$};
% \node[subdag,draw=black] (inc) at (3,-3) {$T_3$};
% % \draw[->] (y) -- (z);

% \branches{z}{gt.north}{eq.north}{inc.north}
% \end{tikzpicture}
% \end{minipage}\begin{minipage}{.5\linewidth}
% \begin{tikzpicture}[inner sep=2pt,subdag/.style = { regular polygon, regular polygon sides=3 }]
% % \node[termnode,processed] (y) at (3,0) {$M$};
% \node[weightnode] (z) at (1.5,-1) {$p$};
% \node[subdag,draw=black] (gt) at (0,-3) {$T_1$};
% \node[subdag,draw=black] (eq) at (1.5,-3) {$T_2$};
% \node[subdag,draw=black] (inc) at (3,-3) {$T_3$};
% % \draw[->] (y) -- (z);
% \gtbranch[]{z}{gt.north};
% \eqbranch[bend right]{z}{inc.north};
% \incbranch[bend left]{z}{inc.north};
% \end{tikzpicture}
% \end{minipage}


% If $s=f(s_1,...,s_n)$, $t=g(t_1,...,t_m)$ and $f\gg g$ and $p=|s|-|t|$.

% \begin{minipage}{.5\linewidth}
% \begin{tikzpicture}[inner sep=2pt,subdag/.style = { regular polygon, regular polygon sides=3 }]
% % \node[termnode,processed] (y) at (3,0) {$M$};
% \node[termnode] (z) at (1.5,-1) {$s\comp t$};
% \node[subdag,draw=black] (gt) at (0,-3) {$T_1$};
% \node[subdag,draw=black] (eq) at (1.5,-3) {$T_2$};
% \node[subdag,draw=black] (inc) at (3,-3) {$T_3$};
% % \draw[->] (y) -- (z);

% \branches{z}{gt.north}{eq.north}{inc.north}
% \end{tikzpicture}
% \end{minipage}\begin{minipage}{.5\linewidth}
% \begin{tikzpicture}[inner sep=2pt,subdag/.style = { regular polygon, regular polygon sides=3 }]
% % \node[termnode,processed] (y) at (3,0) {$M$};
% \node[weightnode] (z) at (1.5,-1) {$p$};
% \node[subdag,draw=black] (gt) at (0,-3) {$T_1$};
% \node[subdag,draw=black] (eq) at (1.5,-3) {$T_2$};
% \node[subdag,draw=black] (inc) at (3,-3) {$T_3$};
% % \draw[->] (y) -- (z);
% \gtbranch[bend right]{z}{gt.north};
% \eqbranch[bend left]{z}{gt.north};
% \incbranch[]{z}{inc.north};
% \end{tikzpicture}
% \end{minipage}


% If $s=f(s_1,...,s_n)$, $t=f(t_1,...,t_n)$ and $p=|s|-|t|$.

% \begin{minipage}{.5\linewidth}
% \begin{tikzpicture}[inner sep=2pt,subdag/.style = { regular polygon, regular polygon sides=3 }]
% % \node[termnode,processed] (y) at (3,0) {$M$};
% \node[termnode] (z) at (1.5,-1) {$s\comp t$};
% \node[subdag,draw=black] (gt) at (0,-3) {$T_1$};
% \node[subdag,draw=black] (eq) at (1.5,-3) {$T_2$};
% \node[subdag,draw=black] (inc) at (3,-3) {$T_3$};
% % \draw[->] (y) -- (z);

% \branches{z}{gt.north}{eq.north}{inc.north}
% \end{tikzpicture}
% \end{minipage}\begin{minipage}{.5\linewidth}
% \begin{tikzpicture}[inner sep=2pt,subdag/.style = { regular polygon, regular polygon sides=3 }]
% % \node[termnode,processed] (y) at (3,0) {$M$};
% \node[weightnode] (z0) at (.5,-1) {$p$};
% \node[termnode] (z1) at (1.5,-1.8) {$s_1\comp t_1$};
% \node[] (z2) at (2.25,-2.4) {};
% \node[termnode] (z3) at (3,-3) {$s_n\comp t_n$};
% \node[subdag,draw=black] (gt) at (0,-4.5) {$T_1$};
% \node[subdag,draw=black] (eq) at (1.5,-4.5) {$T_2$};
% \node[subdag,draw=black] (inc) at (3,-4.5) {$T_3$};
% % \draw[->] (y) -- (z);
% \gtbranch[]{z0}{gt.north};
% \eqbranch[]{z0}{z1};
% \incbranch[bend right]{z0}{inc.north};

% \gtbranch[]{z1}{gt.north};
% \eqbranch[]{z1}{z2};
% \incbranch[bend right]{z1}{inc.north};

% \eqbranch[]{z2}{z3};

% \gtbranch[]{z3}{gt.north};
% \eqbranch[]{z3}{eq.north};
% \incbranch[]{z3}{inc.north};
% \end{tikzpicture}
% \end{minipage}


% \begin{Definition}[Ordering constraints]
% An \emph{atomic ordering constraint} is of the form $s>t$ or $s=t$ where $s,t\in\Terms$, or of the form $p>0$ or $p\gtrsim 0$ where $p\in\Poly$. An \emph{ordering constraint} is a quantifier-free formula built out of atomic ordering constraints and the logical connectives $\neg$, $\land$ and $\lor$. We denote the empty conjunction of constraints with $\top$, $s>t\lor s=t$ with $s\geq t$ and $\neg(s\geq t)$ with $s\ngeq t$.\qed
% \end{Definition}
% %
% Note that we are considering possibly non-ground substitutions, which allows for negations of ordering constraints, such as $s\ngeq t$.
% %
% \begin{Definition}[Ordering constraint semantics]
% Let $\theta$ be a substitution. $\theta$ satisfies the constraint $s>t$ or $s=t$ if $s\theta\succ t\theta$ or $s\theta= t\theta$, respectively. $\theta$ satisfies the constraint $p>0$ or $p\gtrsim 0$ if $\sigma_\theta(p)>0$ or $\sigma_\theta(p)\gtrsim 0$, respectively. Moreover, $\theta$ satisfies the ordering constraints $\neg F$ if it does not satisfy $F$, satisfies $F\land G$ if it satisfies both $F$ and $G$, and satisfies $F\lor G$ if satisfies either $F$ or $G$.\qed
% \end{Definition}
% %
% We assign ordering constraints to edges and paths in an ordering diagram as follows.
% %
% \begin{Definition}
% Let $\Omega=(V,E,r)$ be an ordering diagram. Each edge $v\lto{\ell}w\in E$ is labeled by an ordering constraint, given by $\constraint(v\lto{\ell}w)$.
% \begin{enumerate}[label=(\arabic*)]
% \item If $\lbl(v)=\DATA$, then $\constraint(v\lto{\ell}w)=\top$,
% \item If $\lbl(v)=\COMP$, then let $s=\lhs(v)$ and $t=\rhs(v)$:
% \begin{align*}
% \constraint(e)=\begin{cases}
% s>t, &\text{if }\ell=\gt,\\
% s=t, &\text{if }\ell=\eq,\\
% s\ngeq t, &\text{if }\ell=\nge,
% \end{cases}
% \end{align*}
% \item If $\lbl(v)=\POLY$, then let $p = \poly(v)$:
% \begin{align*}
% \constraint(e)=\begin{cases}
% p > 0, &\text{if }\ell=\gt,\\
% p \gtrsim 0\land p\not> 0, &\text{if }\ell=\eq,\\
% p \not\gtrsim 0, &\text{if }\ell=\nge.
% \end{cases}
% \end{align*}
% \end{enumerate}
% Let $P=v_1\lto{\ell_1} ...\lto{\ell_{n-1}} v_n$ be a path in $\Omega$. We define the ordering constraint corresponding to $P$ as $\constraint(P)=\bigwedge_{i} \constraint(v_i\lto{\ell_i}v_{i+1})$. Given a substitution $\theta$, a path $P$ in $\Omega$ is \emph{satisfied} if $\theta$ satisfies $\constraint(P)$.\qed
% \end{Definition}
% %
% Note that for each substitution $\theta$ and an ordering diagram $\Omega$, there is only one satisfied path to a fail node.

% Let $\Omega_1=(V_1,E_1,r_1,f_1)$ and $\Omega_2=(V_2,E_2,r_2,f_2)$ be two ordering diagrams. The insertion of $\Omega_2$ into $\Omega_1$ is the following ordering diagram:
% $$\Omega'=(V_1\setminus\{f_1\}\cup V_2,E_1\setminus\delta^-(f_1)\cup E_2\cup\{(x,r_2)\mid (x,f_1)\in E_1\},r_1,f_2)$$

% \begin{algorithm}
% \caption{Constraint creation}
% \begin{algorithmic}[1]
% \Func{\constraint}{$v, \ell$}{$C$}
% \Switch{$\lbl(v)$}
%     \Case{$\DATA$}
%         \State \Return $\top$
%     \EndCase
%     \Case{$\COMP$}
%         \State $s\gets\lhs(v);\ t\gets\rhs(v)$
%         \Switch{$\ell$}
%             \Case{$\gt$} \Return $s\succ t$
%             \EndCase
%             \Case{$\eq$} \Return $s=t$
%             \EndCase
%             \Case{$\nge$} \Return $s\nsucceq t$
%             \EndCase
%         \EndSwitch
%     \EndCase
%     \Case{$\POLY$}
%         \State $p\gets\poly(v)$
%         \Switch{$\ell$}
%             \Case{$\gt$} \Return $p>0$
%             \EndCase
%             \Case{$\eq$} \Return $p\gtrsim 0\land p\not>0$
%             \EndCase
%             \Case{$\nge$} \Return $p\not\gtrsim 0$
%             \EndCase
%         \EndSwitch
%     \EndCase
% \EndSwitch
% \EndFunc
% \end{algorithmic}
% \end{algorithm}

\begin{center}
\begin{tikzpicture}[scale=0.7]
\begin{dot2tex}[codeonly,tikz,options=-t raw]

digraph {
nodesep = 0;
sep = 0;
ranksep = 0;
esep = 0;
source [style = invisible, label = ""];
n0 [
  style = "processed,termnode,"
  label = "$x \comp y$"
];
n1 [
  style = "processed,datanode,"
  label = "1"
];
n2 [
  style = "processed,termnode,"
  label = "$y \comp z$"
];
n3 [
  style = "processed,termnode,"
  label = "$x \comp z$"
];
n4 [
  style = "processed,termnode,"
  label = "$x \comp z$"
];
n5 [
  style = "processed,datanode,"
  label = "1"
];
n6 [
  style = "processed,sinknode,"
  label = ""
];
n7 [
  style = "processed,datanode,"
  label = "2"
];
n8 [
  style = "processed,termnode,"
  label = "$y \comp x$"
];
n9 [
  style = "processed,datanode,"
  label = "2"
];
n10 [
  style = "processed,datanode,"
  label = "2"
];
n11 [
  style = "processed,datanode,"
  label = "2"
];
n12 [
  style = "termnode,"
  label = "$z \comp y$"
];
n13 [
  style = "datanode,"
  label = "2"
];

source -> n0 [style = trueedge];
n0 -> n1 [style = gtedge];
n0 -> n2 [style = eqedge];
n0 -> n3 [style = ngeedge];
n1 -> n4 [style = trueedge];
n2 -> n5 [style = gtedge];
n2 -> n6 [style = eqedge];
n2 -> n6 [style = ngeedge];
n3 -> n7 [style = gtedge];
n3 -> n8 [style = eqedge];
n3 -> n6 [style = ngeedge];
n4 -> n9 [style = gtedge];
n4 -> n6 [style = eqedge];
n4 -> n6 [style = ngeedge];
n5 -> n10 [style = trueedge];
n7 -> n6 [style = trueedge];
n8 -> n11 [style = gtedge];
n8 -> n12 [style = eqedge];
n8 -> n6 [style = ngeedge];
n9 -> n6 [style = trueedge];
n10 -> n6 [style = trueedge];
n11 -> n6 [style = trueedge];
n12 -> n13 [style = gtedge];
n12 -> n6 [style = eqedge];
n12 -> n6 [style = ngeedge];
n13 -> n6 [style = trueedge];
}

\end{dot2tex}
\end{tikzpicture}
\end{center}


\section*{Appendix}
\label{sec:appendix}

\subsection*{Example \ref{ex:traverse} continued}

\begin{center}
\begin{tikzpicture}
\node[] (source) at (0,.7) {};
\node[termnode=left:1.2,processed] (c12) at (0,0) {$x\comp y$};
\node[termnode=above:1.3.2,processed] (c132) at (-1.5,-1) {$y\comp z$};
\node[datanode=left:2] (s1) at (0,-2) {$s\eqs t$};
\node[termnode=above:3] (c2) at (2,0) {$s\comp u$};
\node[datanode=above right:4] (s2) at (2,-2) {$s\eqs u$};

\altbranch{source}{c12};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c132};
\incbranch[]{c12}{c2};

\gtbranch[]{c132}{s1};
\eqbranch[]{c132}{c2};
\incbranch[bend right=15]{c132}{c2};

\gtbranch[]{c2}{s2};

\altbranch[]{s1}{c2};

\begin{scope}[on background layer]
\draw[traceedge,line cap=round] (source) edge (c12);
\node[currtermnode] at (c12) {$x\comp y$};
\draw[traceedge] (c12) edge (c132);
\node[currtermnode] at (c132) {$y\comp z$};
\draw[traceedge] (c132) edge (c2);
\node[currtermnode] at (c2) {$s\comp u$};
\end{scope}

\end{tikzpicture}
\end{center}


\begin{center}
\begin{tikzpicture}
\node[] (source) at (0,.7) {};
\node[termnode=left:1.2,processed] (c12) at (0,0) {$x\comp y$};
\node[termnode=above left:1.3.2,processed] (c132) at (-1.5,-1) {$y\comp z$};
\node[datanode=left:2] (s1) at (0,-2) {$s\eqs t$};
\node[polynode=above:3.1] (c21) at (1,1) {$p\comp p$};
\node[termnode=above:3.2] (c22) at (2,0) {$x\comp z$};
\node[termnode=above:3.3] (c23) at (3,-1) {$s'\comp u'$};
\node[datanode=right:4] (s2) at (2,-2) {$s\eqs u$};

\altbranch{source}{c12};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c132};
\incbranch[]{c12}{c21};

\gtbranch[]{c132}{s1};
\eqbranch[bend right=60]{c132.east}{c21};
\incbranch[bend left=30]{c132}{c21};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};

\gtbranch[]{c22}{s2};
\eqbranch[]{c22}{c23};

\gtbranch[]{c23}{s2};

\altbranch[]{s1}{c21};

\begin{scope}[on background layer]
\draw[traceedge,line cap=round] (source) edge (c12);
\node[currtermnode] at (c12) {$x\comp y$};
\draw[traceedge] (c12) edge (c132);
\node[currtermnode] at (c132) {$y\comp z$};
\draw[traceedge,bend right=60] (c132.east) edge (c21);
\node[currpolynode] at (c21) {$p\comp p$};
\end{scope}

\end{tikzpicture}
\end{center}


\begin{center}
\begin{tikzpicture}
\node[] (source) at (0,.7) {};
\node[termnode=left:1.2,processed] (c12) at (0,0) {$x\comp y$};
\node[termnode=above left:1.3.2,processed] (c132) at (-1.5,-1) {$y\comp z$};
\node[datanode=left:2] (s1) at (0,-2) {$s\eqs t$};
\node[polynode=above:3.1] (c21) at (1,1) {$p\comp p$};
\node[termnode=above:3.2] (c22) at (2,0) {$x\comp z$};
\node[termnode=above:3.3] (c23) at (3,-1) {$s'\comp u'$};
\node[datanode=right:4] (s2) at (2,-2) {$s\eqs u$};

\altbranch{source}{c12};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c132};
\incbranch[]{c12}{c21};

\gtbranch[]{c132}{s1};
\eqbranch[]{c132}{c22};
\incbranch[bend left=30]{c132}{c21};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};

\gtbranch[]{c22}{s2};
\eqbranch[]{c22}{c23};

\gtbranch[]{c23}{s2};

\altbranch[]{s1}{c21};

\begin{scope}[on background layer]
\draw[traceedge,line cap=round] (source) edge (c12);
\node[currtermnode] at (c12) {$x\comp y$};
\draw[traceedge] (c12) edge (c132);
\node[currtermnode] at (c132) {$y\comp z$};
\draw[traceedge] (c132) edge (c22);
\node[currtermnode] at (c22) {$x\comp z$};
\end{scope}

\end{tikzpicture}
\end{center}


\begin{center}
\begin{tikzpicture}
\node[] (source) at (0,.7) {};
\node[termnode=left:1.2,processed] (c12) at (0,0) {$x\comp y$};
\node[termnode=above left:1.3.2,processed] (c132) at (-1.5,-1) {$y\comp z$};
\node[datanode=left:2] (s1) at (0,-2) {$s\eqs t$};
\node[polynode=above:3.1] (c21) at (1,1) {$p\comp p$};
\node[termnode=above:3.2] (c22) at (2,0) {$x\comp z$};
\node[termnode=above:3.3] (c23) at (3,-1) {$s'\comp u'$};
\node[datanode=right:4] (s2) at (2,-2) {$s\eqs u$};

\altbranch{source}{c12};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c132};
\incbranch[]{c12}{c21};

\gtbranch[]{c132}{s1};
\eqbranch[]{c132}{c23};
\incbranch[bend left=30]{c132}{c21};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};

\gtbranch[]{c22}{s2};
\eqbranch[]{c22}{c23};

\gtbranch[]{c23}{s2};

\altbranch[]{s1}{c21};

\begin{scope}[on background layer]
\draw[traceedge,line cap=round] (source) edge (c12);
\node[currtermnode] at (c12) {$x\comp y$};
\draw[traceedge] (c12) edge (c132);
\node[currtermnode] at (c132) {$y\comp z$};
\draw[traceedge] (c132) edge (c23);
\node[currtermnode] at (c23) {$s'\comp u'$};
\end{scope}

\end{tikzpicture}
\end{center}

\begin{center}
\begin{tikzpicture}
\node[] (source) at (0,.7) {};
\node[termnode=left:1.2,processed] (c12) at (0,0) {$x\comp y$};
\node[termnode=above left:1.3.2,processed] (c132) at (-1.5,-1) {$y\comp z$};
\node[datanode=left:2] (s1) at (0,-2) {$s\eqs t$};
\node[polynode=above:3.1] (c21) at (1,1) {$p\comp p$};
\node[termnode=above:3.2] (c22) at (2,0) {$x\comp z$};
\node[termnode=above:3.3.1] (c231) at (3,-1) {$y\comp x$};
\node[termnode=above:3.3.2] (c232) at (4,-2) {$z\comp y$};
\node[datanode=below right:4] (s2) at (2,-2) {$s\eqs u$};

\altbranch{source}{c12};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c132};
\incbranch[]{c12}{c21};

\gtbranch[]{c132}{s1};
\eqbranch[]{c132}{c231};
\incbranch[bend left=30]{c132}{c21};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};

\gtbranch[]{c22}{s2};
\eqbranch[]{c22}{c231};

\gtbranch[]{c231}{s2};
\eqbranch[]{c231}{c232};

\gtbranch[]{c232}{s2};

\altbranch[]{s1}{c21};

\begin{scope}[on background layer]
\draw[traceedge,line cap=round] (source) edge (c12);
\node[currtermnode] at (c12) {$x\comp y$};
\draw[traceedge] (c12) edge (c132);
\node[currtermnode] at (c132) {$y\comp z$};
\draw[traceedge] (c132) edge (c231);
\node[currtermnode] at (c231) {$y\comp x$};
\end{scope}

\end{tikzpicture}
\end{center}


\begin{center}
\begin{tikzpicture}
\node[] (source) at (0,.7) {};
\node[termnode=left:1.2,processed] (c12) at (0,0) {$x\comp y$};
\node[termnode=above left:1.3.2,processed] (c132) at (-1.5,-1) {$y\comp z$};
\node[datanode=left:2] (s1) at (0,-2) {$s\eqs t$};
\node[polynode=above:3.1] (c21) at (1,1) {$p\comp p$};
\node[termnode=above:3.2] (c22) at (2,0) {$x\comp z$};
\node[termnode=above:3.3.1] (c231) at (3,-1) {$y\comp x$};
\node[termnode=above:3.3.2] (c232) at (4,-2) {$z\comp y$};
\node[datanode=below right:4] (s2) at (2,-2) {$s\eqs u$};

\altbranch{source}{c12};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c132};
\incbranch[]{c12}{c21};

\gtbranch[]{c132}{s1};
\eqbranch[bend left=10]{c132}{c232};
\incbranch[bend left=30]{c132}{c21};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};

\gtbranch[]{c22}{s2};
\eqbranch[]{c22}{c231};

\gtbranch[]{c231}{s2};
\eqbranch[]{c231}{c232};

\gtbranch[]{c232}{s2};

\altbranch[]{s1}{c21};

\begin{scope}[on background layer]
\draw[traceedge,line cap=round] (source) edge (c12);
\node[currtermnode] at (c12) {$x\comp y$};
\draw[traceedge] (c12) edge (c132);
\node[currtermnode] at (c132) {$y\comp z$};
\draw[traceedge,bend left=10] (c132) edge (c232);
\node[currtermnode] at (c232) {$z\comp y$};
\end{scope}

\end{tikzpicture}
\end{center}


\begin{center}
\begin{tikzpicture}
\node[] (source) at (0,.7) {};
\node[termnode=left:1.2,processed] (c12) at (0,0) {$x\comp y$};
\node[termnode=above left:1.3.2,processed] (c132) at (-1.5,-1) {$y\comp z$};
\node[datanode=left:2] (s1) at (0,-2) {$s\eqs t$};
\node[polynode=above:3.1] (c21) at (1,1) {$p\comp p$};
\node[termnode=above:3.2] (c22) at (2,0) {$x\comp z$};
\node[termnode=above:3.3.1] (c231) at (3,-1) {$y\comp x$};
\node[termnode=above:3.3.2] (c232) at (4,-2) {$z\comp y$};
\node[datanode=below right:4] (s2) at (2,-2) {$s\eqs u$};
\node[sinknode] (sink) at (-1.5,-2) {};

\altbranch{source}{c12};

\gtbranch[]{c12}{s1};
\eqbranch[]{c12}{c132};
\incbranch[]{c12}{c21};

\gtbranch[]{c132}{s1};
\eqbranch[]{c132}{sink};
\incbranch[bend left=30]{c132}{c21};

\gtbranch[]{c21}{s2};
\eqbranch[]{c21}{c22};

\gtbranch[]{c22}{s2};
\eqbranch[]{c22}{c231};

\gtbranch[]{c231}{s2};
\eqbranch[]{c231}{c232};

\gtbranch[]{c232}{s2};

\altbranch[]{s1}{c21};

\begin{scope}[on background layer]
\draw[traceedge,line cap=round] (source) edge (c12);
\node[currtermnode] at (c12) {$x\comp y$};
\draw[traceedge] (c12) edge (c132);
\node[currtermnode] at (c132) {$y\comp z$};
\draw[traceedge] (c132) edge (sink);
\node[currpolynode,circle,inner sep=4pt] at (sink) {};
\end{scope}

\end{tikzpicture}
\end{center}

%

\begin{Definition}[Path Equivalence]
Let $p=v_1\to\ldots\to v_n$ and $q=w_1\to\ldots\to w_n$ be two paths. We say $p$ and $q$ are \emph{equivalent} and write $p\sim q$ if $v_i$ and $w_i$ have identical labels for $1\le i\le n$.
Let $\OD$ and $\ODprime$ be TODs.\qed
\end{Definition}
%
The following lemma is used in correctness proofs of our algorithms. 
%
\begin{lemma}[TOD Equivalence]
\label{lem:ordering-diagram-equivalence}
Let $\OD$ and $\ODprime$ be two well-formed TODs. Then $\OD\sim\ODprime$ if for each substitution $\theta$, there are nodes $v$, $v'$, $w$ and $w'$ and $D\in Seq(\mathcal{D})$ s.t. $\trace(\OD,\theta)$ and $\trace(\ODprime,\theta)$ are of the form $$v_1\to\ldots\to v_n\to v\to\ldots\to v'\to v'_1\to\ldots\to v'_m\text{ and }$$
$$w_1\to\ldots\to w_n\to w\to\ldots\to w'\to w'_1\to\ldots\to w'_m,$$
for some $n,m\geq 0$, respectively, and
\begin{enumerate}[label=(\arabic*)]
\item $(v_1\to\ldots\to v_n)\sim(w_1\to\ldots\to w_n)$,
\item $(v'\to v'_1\to\ldots\to v'_m)\sim(w'\to w'_1\to\ldots\to w'_m)$,
\item $\phi(v,\theta)=D\cons \phi(v',\theta)$ and $\phi(w,\theta)=D\cons \phi(w',\theta)$.
\end{enumerate}
\end{lemma}
\begin{proof}
Since $v_1=\src(\OD)$ and $w_1=\src(\ODprime)$, we have to prove that $\phi(v_1,\theta)=\phi(w_1,\theta)$.
First, we prove that $\phi(v'_i,\theta)=\phi(w'_i,\theta)$ for all $0\le i\le m$ by induction on $m-i$. If $m-i=0$, then $v'_i=v'_m=\snk(\OD)$ and $w'_i=w'_m=\snk(\ODprime)$, and the claim follows trivially. Otherwise, $m-i>0$. If $\lbl(v'_i)=\DATA{}$, then $\lbl(w'_i)=\DATA$ by (1) as well and we have
$$\phi(v'_i,\theta)=\langle d\rangle\cons\phi(v'_{i+1},\theta)=\langle d\rangle\cons\phi(w'_{i+1},\theta)=\phi(w'_i,\theta)$$
by the induction hypothesis where $d=\data(v'_i)=\data(w'_i)$ by (1). Otherwise,
$$\phi(v'_i,\theta)=\phi(v'_{i+1},\theta)=\phi(w'_{i+1},\theta)=\phi(w'_i,\theta),$$
since $\nextF(v'_i,\theta)=v'_{i+1}$ and $\nextF(w'_i,\theta)=w'_{i+1}$ by definition of the trace. Hence, $\phi(v'_1,\theta)=\phi(w'_1,\theta)$. Using this and a similar argument, we get $\phi(v',\theta)=\phi(w',\theta)$ and from (2), we get that $\phi(v,\theta)=\phi(w,\theta)$. Finally, using (3), we prove that $\phi(v_i,\theta)=\phi(w_i,\theta)$ for all $1\le i\le n$ by induction on $n-i$, similarly to the first part, which proves $\phi(v_1,\theta)=\phi(w_1,\theta)$.\qed
\end{proof}

\expandCorrectness*
\begin{proof}
Let $\OD$ and $u\lto{\ell}v$ be an ordering diagram and an edge that satisfy the input conditions of $\expand{}$. We prove the claim by induction on $\OD$ w.r.t. the well-founded ordering $\gtrdot$. The induction hypothesis is that for all ordering diagrams $\OD'$ and edges $u'\lto{\ell'} v'$ satisfying the preconditions of \expand{} and $\OD\gtrdot\OD'$, $\expand(\OD',u'\lto{\ell'}v')$ is correct.

If $\proc(v)$, then $w=v$ and $\OD=\ODprime$, so the claim follows trivially. Otherwise, let $\ODprime$ and $u'\lto{\ell'}v'$ be the ordering diagram and node corresponding to $\OD$ and $u\lto{\ell}v$ after executing the loop body once. First, we verify that the loop body preserves well-formedness, since it only performs function calls or operations that preserve this property. Now we prove $\OD\sim\ODprime$ and $\OD\gtrdot\ODprime$. Let $\kay$ be the output of $\inferPath(\OD,u\lto{\ell}v)$. Note that the preconditions of \inferPath are satisfied by $\OD$ and $u\lto{\ell}v$, so we the post-condition holds. We have the following cases:
%
\begin{enumerate}[label=(\arabic*)]
\item $\kay\neq\true$. It follows from the post-condition of \inferPath that $\lbl(v)$ is either \TERM{} or \POLY{}. We now apply Lemma~\ref{lem:ordering-diagram-equivalence} to prove $\OD\sim\ODprime$. Let $\theta$ be an arbitrary substitution and we distinguish two cases. If $u\lto{\ell}v\notin\trace(\OD,\theta)$, then since lines 7-8 of \expand{} do not modify any edges or nodes apart from $u$ and its outgoing edges, $\trace(\OD,\theta)\sim\trace(\ODprime,\theta)$ and we are done.

Otherwise, $u\lto{\ell}v\in\trace(\OD,\theta)$. In this case, the two traces are of the form $\ldots\to u\to v\to w\to\ldots$ and $\ldots\to u'\to v'\to\ldots$. By the post-conditions of \inferPath, $w=\kay(v)$, so $(\ldots\to u)\sim(\ldots \to u')$ and $(\kay(v)\to\ldots)\sim(v'\to\ldots)$. We only have to prove $\phi(v,\theta)=D\cons\phi(\kay(v),\theta)$ and $\phi(v',\theta)=D\cons\phi(v',\theta)$ for some $D\in Seq(\mathcal{D})$. This follows by taking $D=\langle\rangle$ and from the fact that $\lbl(v)$ is either \TERM{} or \POLY{}. We also have that $u'\lto{\ell'}v'\in E(\ODprime)$ and $\proc(u')$, moreover, $\OD>\ODprime$ since we have one less edge in $\ODprime$ compared to $\OD$.

\item If $\kay=\true$ and $\isFuncComp(v)$, then $\ODprime=\expandFunc(\OD,v)$. The preconditions of \expandFunc{} hold, so $\OD\sim \ODprime$ and $\OD>\ODprime$.

\item If $\kay=\true$ and $\neg\isFuncComp(v)$. Again, we apply Lemma~\ref{lem:ordering-diagram-equivalence}. Let $\theta$ be an arbitrary substitution. We only have to check $u\lto{\ell}v\in\trace(\OD,\theta)$, as otherwise the claim follows trivially. The two traces are of the form $\ldots\to u\to v\to w\to\ldots$ and $\ldots\to u'\to v'\to w'\to\ldots$ where $(\ldots\to u)\sim(\ldots \to u')$ and $(w\to\ldots)\sim(w'\to\ldots)$. It remains to prove that $\phi(v,\theta)=D\cons\phi(w,\theta)$ and $\phi(v',\theta)=D\cons\phi(w',\theta)$ for some $D\in Seq(\mathcal{D})$. Except for $\proc(v)\neq\proc(w)$, $w$ has the same labels as $v$ and the same outgoing edges, this holds as well.
\end{enumerate}
%
We have proved $\OD\sim\ODprime$ and $\OD\gtrdot\ODprime$, and by the input conditions of \expand{} and the induction hypothesis, the call $\expand(\ODprime,u'\lto{\ell'}v')$ results in a pair that satisfies the output conditions.\qed
\end{proof}

\expandFuncKBOCorrectness*

\begin{proof}
Let $\OD$ be a well-formed ordering diagram and $v$ a node which satisfy the requirements of $\expandFunc_\kbo$. Let $(\ODprime,w)$ be the output of the call $\expandFunc_\kbo(\OD,v)$. We first argue that $\ODprime$ is well-formed.
%
\begin{enumerate}[label=(\arabic*),itemsep=2pt,parsep=2pt]
\item $\ODprime$ is acyclic, since $\OD$ is acyclic and we only added new edges from $v$ or fresh nodes to $\gt(v)$, $\eq(v)$ and $\nge(v)$ on lines 6, 8, 13 and 15, or from $v$ or a previously added node to a currently added fresh node on line 13. $\proc(\ODprime)$ is also a tree, since $\neg\proc(v)$, none of its successors, nor the fresh nodes are processed, so $\proc(\OD)$ is isomorphic to $\proc(\ODprime)$. This proves~\ref{prop:well-formed1}.
\item $\ODprime$ has one \SOURCE{} and \SINK{} node and $\proc(\src(\ODprime))$, since these parts were not modified by the call, hence we have~\ref{prop:well-formed2}.
\item the \gt{} and \nge{} edges of $w$ remain intact, while the \eq{} edge is removed on line 5, and either added back at line 7, 9, 14 or 16. The \gt{} and \nge{} edges of new nodes are set on line 14, and their \eq{} edges are set of line 14 or 16. This proves~\ref{prop:well-formed3}.
\item $\lhsT(w)$ and $\rhsT(w)$ are set on line 17 while $\lhsT(v)$ and $\rhsT(v)$ are set for new nodes on line 13. This proves~\ref{prop:well-formed4}.
\end{enumerate}
Hence $\ODprime$ is well-formed. Evidently, $w\in V(\ODprime)$. \todo{Find order for $v>w$ and prove it.} We now prove $\OD\sim\ODprime$. Let $\theta$ be an arbitrary substitution. Let us denote with $w_\gt$, $w_\eq$ and $w_\nge$ the nodes in $\ODprime$ corresponding to the nodes $\gt(v)$, $\eq(v)$ and $\nge(v)$ in $\OD$, respectively. Note that the function does not modify any nodes or outgoing edges in $V(G)\setminus \{v\}$, so we can assume that $\phi(\gt(v),\theta)=\phi(w_\gt,\theta)$, $\phi(\eq(v),\theta)=\phi(w_\eq,\theta)$ and $\phi(\nge(v),\theta)=\phi(w_\nge,\theta)$, and we only have to verify that $\phi(v,\theta)=\phi(w,\theta)$. We consider the following cases:
\begin{enumerate}[label=(\arabic*),itemsep=2pt,parsep=2pt]
\item $\sigma_\theta(|s|)>\sigma_\theta(|t|)$. Then by~\ref{prop:kbo1}, $\nextF(v,\theta)=\gt$, $\nextF(w,\theta)=\gt$ and by construction, $\gt(w)=w_\gt$, hence
$$\phi(v,\theta)=\phi(\gt(v),\theta)=\phi(w_\gt,\theta)=\phi(\gt(w),\theta)=\phi(w,\theta).$$
\item $\sigma_\theta(|s|)\not\gtrsim\sigma_\theta(|t|)$. Then none of~\ref{prop:kbo1}--\ref{prop:kbo3} applies, so $\nextF(v,\theta)=\nge$, $\nextF(w,\theta)=\nge$ and by construction, $\nge(w)=w_\nge$, hence
$$\phi(v,\theta)=\phi(\nge(v),\theta)=\phi(w_\nge,\theta)=\phi(\nge(w),\theta)=\phi(w,\theta).$$
\item $\sigma_\theta(|s|)\gtrsim\sigma_\theta(|t|)$ and $f\gg g$. Then by~\ref{prop:kbo2}, $\nextF(v,\theta)=\gt$, $\nextF(w,\theta)=\eq$ and by construction $\eq(v)=w_\gt$, hence
$$\phi(v,\theta)=\phi(\gt(v),\theta)=\phi(w_\gt,\theta)=\phi(\eq(w),\theta)=\phi(w,\theta).$$
\item $\sigma_\theta(|s|)\gtrsim\sigma_\theta(|t|)$ and $g\gg f$. Then none of~\ref{prop:kbo1}--\ref{prop:kbo3} applies, so $\nextF(v,\theta)=\nge$, $\nextF(w,\theta)=\eq$ and by construction $\eq(w)=w_\nge$, hence
$$\phi(v,\theta)=\phi(\nge(v),\theta)=\phi(w_\nge,\theta)=\phi(\eq(w),\theta)=\phi(w,\theta).$$
\item $\sigma_\theta(|s|)\gtrsim\sigma_\theta(|t|)$ and $f=g$. Then there are exactly $n$ new nodes $w_1,...,w_n$ s.t. by construction $\eq(w)=w_1$, $\eq(w_1)=w_2$, $\ldots$, $\eq(w_{n-1})=w_n$. We consider the following subcases:
\begin{enumerate}[label=(5.\arabic*),leftmargin=.7em]
    \item There is some $1\le i\le n$ s.t. $s_j\theta=t_j\theta$ for all $1\le j < i$ and $s_i\theta\succ_\kbo t_i\theta$. Then by~\ref{prop:kbo3}, $\nextF(v,\theta)=\gt$, $\nextF(w,\theta)=\eq$, $\nextF(w_j,\theta)=\eq$ for all $1\le j < i$ and $\nextF(w_i,\theta)=\gt$. By construction, $\gt(w_i)=w_\gt$ and hence
    \begin{align*}\phi(v,\theta)=\phi(\gt(v),\theta)=\phi(w_\gt,\theta)&=\phi(\gt(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\eq(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\eq(w_1),\theta)=\phi(w_1,\theta)\\
    &=\phi(\eq(w),\theta)=\phi(w,\theta).\end{align*}
    \item There is some $1\le i\le n$ s.t. $s_j\theta=t_j\theta$ for all $1\le j < i$ and $s_i\theta\nsucceq_\kbo t_i\theta$. Then none of~\ref{prop:kbo1}--\ref{prop:kbo3} applies, so $\nextF(v,\theta)=\nge$, $\nextF(w,\theta)=\eq$, $\nextF(w_j,\theta)=\eq$ for all $1\le j < i$ and $\nextF(w_i,\theta)=\nge$. By construction, $\nge(w_i)=w_\nge$ and hence
    \begin{align*}\phi(v,\theta)=\phi(\nge(v),\theta)=\phi(w_\nge,\theta)&=\phi(\nge(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\eq(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\eq(w_1),\theta)=\phi(w_1,\theta)\\
    &=\phi(\eq(w),\theta)=\phi(w,\theta).\end{align*}
    \item Otherwise, $s_i\theta=t_i\theta$ for all $1\le i\le n$. Then also $s\theta=t\theta$, so $\nextF(v,\theta)=\eq$, $\nextF(w,\theta)=\eq$, $\nextF(w_i,\theta)=\eq$ for all $1\le i \le n$. By construction, $\eq(w_n)=w_\eq$ and hence
    \begin{align*}\phi(v,\theta)=\phi(\eq(v),\theta)=\phi(w_\eq,\theta)&=\phi(\eq(w_n),\theta)=\phi(w_n,\theta)\\
    &=\phi(\eq(w_{n-1},\theta)=\phi(w_{n-1},\theta)\\
    &\ldots\\
    &=\phi(\eq(w_1),\theta)=\phi(w_1,\theta)\\
    &=\phi(\eq(w),\theta)=\phi(w,\theta).\end{align*}
\end{enumerate}
\end{enumerate}
\qed
\end{proof}

\expandFuncLPOCorrectness*
\begin{proof}
Let $\OD$ be a well-formed ordering diagram and $v$ a node which satisfy the requirements of $\expandFunc_\lpo$. Let $(\ODprime,w)$ be the output of the call $\expandFunc_\lpo(\OD,v)$. We first argue that $\ODprime$ is well-formed.

...

We now prove $\OD\sim\ODprime$. Let $\theta$ be an arbitrary substitution. Similarly to the proof of Theorem~\ref{thm:expandFuncKBO}, let us denote with $w_\gt$, $w_\eq$ and $w_\nge$ the nodes in $\ODprime$ corresponding to the nodes $\gt(v)$, $\eq(v)$ and $\nge(v)$ in $\OD$, respectively and we also note that the function does not modify any nodes in $V(G)\setminus \{v\}$, so we can assume again that $\phi(\gt(v),\theta)=\phi(w_\gt,\theta)$, $\phi(\eq(v),\theta)=\phi(w_\eq,\theta)$ and $\phi(\nge(v),\theta)=\phi(w_\nge,\theta)$, and we only have to verify that $\phi(v,\theta)=\phi(w,\theta)$. We consider the following cases:
\begin{enumerate}[label=(\arabic*),itemsep=2pt,parsep=2pt]
\item $f\gg g$ and $s\theta\succ_\lpo t_i\theta$ for all $1\le i \le m$. Then by~\ref{prop:lpo2}, $\nextF(v,\theta)=\gt$. Let $w_1=w$ and let $w_2,\ldots,w_m$ be the $m-1$ nodes created by the function call to $\allGT$. We have $\gt(w_1)=w_2$, $\gt(w_2)=w_3$, $\ldots$, $\gt(w_{m-1})=w_m$, $\gt(w_m)=w_\gt$. Moreover, $\lhsT(w_1)=\ldots=\lhsT(w_m)=s$ and $\rhsT(w_1)=t_1$, $\ldots$, $\rhsT(w_m)=t_m$, so $\nextF(w_1,\theta)=\ldots=\nextF(w_m,\theta)=\gt$ and hence
\begin{align*}
    \phi(v,\theta)=\phi(\gt(v),\theta)=\phi(w_\gt,\theta)&=\phi(\gt(w_m),\theta)=\phi(w_m,\theta)\\
    &=\phi(\gt(w_{m-1}),\theta)=\phi(w_{m-1},\theta)\\
    &\ldots\\
    &=\phi(\gt(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\gt(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
\item $f\gg g$ and there is some $1\le i\le m$ s.t. $s\theta\succ_\lpo t_j\theta$ for all $1\le j \le i$ and $s\theta\nsucc_\lpo t_i\theta$. \ref{prop:lpo1} and~\ref{prop:lpo2} do not apply, and for all $1\le j\le m$, $s\theta\succ_\lpo s_j\theta$ and $t\theta\succ_\lpo t_i\theta$, so $s_j\theta\succeq_\lpo t\theta$ would contradict $s\theta\nsucc_\lpo t_i\theta$ and hence~\ref{prop:lpo3} does not apply either. This means $\nextF(v,\theta)=\nge$. Similarly to the previous case, let $w_1=w$ and $w_2,\ldots,w_m$ be the nodes created by \allGT{}. We have $\gt(w_1)=w_2$, $\ldots$, $\gt(w_{i-1})=w_i$ and $\nge(w_i)=\eq(w_i)=w_\nge$. Again, $\lhsT(w_1)=\ldots=\lhsT(w_m)=s$ and $\rhsT(w_1)=t_1$, $\ldots$, $\rhsT(w_m)=t_m$, so $\nextF(w_1,\theta)=\ldots=\nextF(w_{i-1},\theta)=\gt$. If $\nextF(w_i,\theta)=\eq$, then
\begin{align*}
    \phi(v,\theta)=\phi(\nge(v),\theta)=\phi(w_\nge,\theta)&=\phi(\eq(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\gt(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\gt(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\gt(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
Otherwise, $\nextF(w_i,\theta)=\nge$ and we get
\begin{align*}
    \phi(v,\theta)=\phi(\nge(v),\theta)=\phi(w_\nge,\theta)&=\phi(\nge(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\gt(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\gt(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\gt(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
\item $g\gg f$ and there is some $1\le i\le n$ s.t. $s_j\theta\nsucceq_\lpo t$ for all $1\le j < i$ and $s_i\theta\succeq_\lpo t\theta$. Then by~\ref{prop:lpo3}, $\nextF(v,\theta)=\gt$.

Let $w_1=w$ and $w_2,\ldots,w_n$ be the nodes created by the call to \someGEQ{}. We have $\nge(w_1)=w_2$, $\nge(w_2)=w_3$, $\ldots$, $\nge(w_{i-1})=w_i$ and $\gt(w_i)=\eq(w_i)=w_\gt$. We also have $\lhsT(w_1)=s_1$, $\ldots$, $\lhsT(w_n)=s_n$ and $\rhsT(w_1)=\ldots=\rhsT(w_n)=t$, so $\nextF(w_1,\theta)=\ldots=\nextF(w_{i-1},\theta)=\nge$. If $\nextF(w_i,\theta)=\gt$, then
\begin{align*}
    \phi(v,\theta)=\phi(\gt(v),\theta)=\phi(w_\gt,\theta)&=\phi(\gt(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\nge(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\nge(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\nge(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
Otherwise, $\nextF(w_i,\theta)=\eq$ and we have
\begin{align*}
    \phi(v,\theta)=\phi(\gt(v),\theta)=\phi(w_\gt,\theta)&=\phi(\eq(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\nge(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\nge(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\nge(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
\item $g\gg f$ and for all $1\le i\le n$, $s_i\theta\nsucceq_\lpo t\theta$. Then none of~\ref{prop:lpo1}--\ref{prop:lpo3} applies, so $\nextF(v,\theta)=\nge$. Again, let $w_1=w$ and $w_2,\ldots,w_n$ be the nodes created by the call to \someGEQ{}. We have $\nge(w_1)=w_2$, $\nge(w_2)=w_3$, $\ldots$, $\nge(w_{n-1})=w_n$, $\nge(w_n)=w_\nge$. We also have $\lhsT(w_1)=s_1$, $\ldots$, $\lhsT(w_n)=s_n$ and $\rhsT(w_1)=\ldots=\rhsT(w_n)=t$, so $\nextF(w_1,\theta)=\ldots=\nextF(w_n,\theta)=\nge$, hence
\begin{align*}
    \phi(v,\theta)=\phi(\nge(v),\theta)=\phi(w_\nge,\theta)&=\phi(\nge(w_n),\theta)=\phi(w_n,\theta)\\
    &=\phi(\nge(w_{n-1}),\theta)=\phi(w_{n-1},\theta)\\
    &\ldots\\
    &=\phi(\nge(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\nge(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
\item $f=g$ and there exists $1\le i\le n$ s.t. $s_j\theta=t_j\theta$ for all $1\le j < i$, $s_i\theta\succ_\lpo t_i\theta$ and $s\theta\succ_\lpo t_k\theta$ for all $i < k \le n$. Then, \ref{prop:lpo1} applies, so $\nextF(v,\theta)=\gt$.

Let $w_1=w$, let $w_2,\ldots,w_i$ be the $i-1$ nodes created up to the $i-1$th iteration in the \textbf{for} loop and let $w_{i+1},\ldots,w_n$ be the $n-i$ nodes created by the function call to \allGT{} in the $i-1$th iteration of the \textbf{for} loop. We have that $\eq(w_1)=w_2$, $\eq(w_2)=w_3$, $\ldots$, $\eq(w_{i-1})=w_i$, $\gt(w_i)=w_{i+1}$, $\gt(w_{i+1})=w_{i+2}$, $\ldots$, $\gt(w_{n-1})=w_n$ and $\gt(w_n)=w_\gt$. We also have $\lhsT(w_1)=s_1$, $\ldots$, $\lhsT(w_i)=s_i$, $\lhsT(w_{i+1})=\ldots=\lhsT(w_n)=s$, $\rhsT(w_1)=t_1$, $\ldots$, $\rhsT(w_n)=t_n$. This means $\nextF(w_1,\theta)=\ldots=\nextF(w_{i-1},\theta)=\eq$, $\nextF(w_i,\theta)=\ldots=\nextF(w_n,\theta)=\gt$. Hence
\begin{align*}
    \phi(v,\theta)=\phi(\gt(v),\theta)=\phi(w_\gt,\theta)&=\phi(\gt(w_n),\theta)=\phi(w_n,\theta)\\
    &=\phi(\gt(w_{n-1}),\theta)=\phi(w_{n-1},\theta)\\
    &\ldots\\
    &=\phi(\gt(w_{i+1}),\theta)=\phi(w_{i+1},\theta)\\
    &=\phi(\gt(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\eq(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\eq(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\eq(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
\item $f=g$ and there exists $1\le i\le n$ and $i<j\le n$ s.t. $s_k\theta=t_k\theta$ for all $1\le k<i$, $s_i\theta\succ_\lpo t_i\theta$, $s\theta\succ_\lpo t_l\theta$ for all $i<l<j$ and $s\theta\nsucc_\lpo t_j\theta$. \ref{prop:lpo1} and \ref{prop:lpo2} do not apply, and for all $1\le k\le m$, $s\theta\succ_\lpo s_k\theta$ and $t\theta\succ_\lpo t_j\theta$, so $s_k\theta\succeq_\lpo t\theta$ would contradict $s\theta\nsucc_\lpo t_j\theta$ and hence~\ref{prop:lpo3} does not apply either. This means $\nextF(v,\theta)=\nge$.

Let $w_1=w$, let $w_2,\ldots,w_i$ be the $i-1$ nodes created up to the $i-1$th iteration in the \textbf{for} loop and let $w_{i+1},\ldots,w_n$ be the $n-i$ nodes created by the function call to \allGT{} in the $i-1$th iteration of the \textbf{for} loop. We have that $\eq(w_1)=w_2$, $\eq(w_2)=w_3$, $\ldots$, $\eq(w_{i-1})=w_i$, $\gt(w_i)=w_{i+1}$, $\gt(w_{i+1})=w_{i+2}$, $\ldots$, $\gt(w_{j-1})=w_j$ and $\eq(w_j)=\nge(w_j)=w_\nge$. We also have $\lhsT(w_1)=s_1$, $\ldots$, $\lhsT(w_i)=s_i$, $\lhsT(w_{i+1})=\ldots=\lhsT(w_j)=s$, $\rhsT(w_1)=t_1$, $\ldots$, $\rhsT(w_j)=t_j$. This means $\nextF(w_1,\theta)=\ldots=\nextF(w_{i-1},\theta)=\eq$, $\nextF(w_i,\theta)=\ldots=\nextF(w_{j-1},\theta)=\gt$. If $\nextF(w_j,\theta)=\eq$, then
\begin{align*}
    \phi(v,\theta)=\phi(\nge(v),\theta)=\phi(w_\nge,\theta)&=\phi(\eq(w_j),\theta)=\phi(w_j,\theta)\\
    &=\phi(\gt(w_{j-1}),\theta)=\phi(w_{j-1},\theta)\\
    &\ldots\\
    &=\phi(\gt(w_{i+1}),\theta)=\phi(w_{i+1},\theta)\\
    &=\phi(\gt(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\eq(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\eq(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\eq(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
Otherwise, $\nextF(w_j,\theta)=\nge$ and hence
\begin{align*}
    \phi(v,\theta)=\phi(\nge(v),\theta)=\phi(w_\nge,\theta)&=\phi(\nge(w_j),\theta)=\phi(w_j,\theta)\\
    &=\phi(\gt(w_{j-1}),\theta)=\phi(w_{j-1},\theta)\\
    &\ldots\\
    &=\phi(\gt(w_{i+1}),\theta)=\phi(w_{i+1},\theta)\\
    &=\phi(\gt(w_i),\theta)=\phi(w_i,\theta)\\
    &=\phi(\eq(w_{i-1}),\theta)=\phi(w_{i-1},\theta)\\
    &\ldots\\
    &=\phi(\eq(w_2),\theta)=\phi(w_2,\theta)\\
    &=\phi(\eq(w_1),\theta)=\phi(w_1,\theta)=\phi(w,\theta).
\end{align*}
\item $f=g$ and there exists $1\le i\le n$ and $i<j\le n$ s.t. $s_k\theta=t_k\theta$ for all $1\le k<i$, $s_i\theta\nsucceq_\lpo t_i\theta$, $s_l\theta\nsucceq_\lpo t\theta$ for all $i<l<j$ and $s_j\theta\succeq_\lpo t\theta$. Since \ref{prop:lpo3} applies, $\nextF(v,\theta)=\gt$. TODO
\item $f=g$ and there exists $1\le i\le n$ s.t. $s_j\theta=t_j\theta$ for all $1\le j<i$, $s_i\theta\nsucceq_\lpo t_i\theta$ and $s_k\theta\nsucceq_\lpo t\theta$ for all $i<k\le n$. \ref{prop:lpo1} and \ref{prop:lpo2} do not apply. Since (a) for all $1\le j<i$, $t\theta\succ_\lpo t_j\theta=s_j\theta$ implies $s_j\theta\nsucceq_\lpo t\theta$, 
(b) $s_i\theta\nsucceq_\lpo t_i\theta$ and $t\theta\succ_\lpo t_i\theta$ implies $s_i\theta\nsucceq_\lpo t\theta$ and (c) for all $i<k\le n$, $s_k\theta\nsucceq_\lpo t\theta$, \ref{prop:lpo3} does not apply either. This means $\nextF(v,\theta)=\nge$. TODO
\item $f=g$ and $s_i\theta=t_i\theta$ for all $1\le i\le n$. \ref{prop:lpo1} and \ref{prop:lpo2} do not apply and for all $1\le i\le n$, $t\theta\succ_\lpo t_i\theta=s_i\theta$ implies $s_i\theta\nsucceq t\theta$, so \ref{prop:lpo3} does not apply either. This means $\nextF(v,\theta)=\eq$. TODO
\end{enumerate}
\qed
\end{proof}

\section*{Miscellaneous algorithms}

\begin{algorithm}[t]
\caption{Ordering diagram miscellaneous algorithms}
\label{alg:miscellaneous}
\algoPreamble
\begin{minipage}{.48\linewidth}

\Fn{$\copyNode(\OD, v)$}{
    $(\OD,w)\gets \newNode(\OD,\lbl(v))$\;
    $\lhsT(w)\gets \lhsT(v)$\;
    $\rhsT(w)\gets \rhsT(v)$\;
    $\lhsP(w)\gets \lhsP(v)$\;
    $\rhsP(w)\gets \rhsP(v)$\;
    $\data(w)\gets \data(v)$\;
    \For{$\ell\in\{\gt,\eq,\nge,\true\}$}{
        \If{$\ell(v)$}{
            $E(\OD)\gets E(\OD)\cup\{w\lto{\ell}\ell(v)\}$
        }
    }
    \Return $(\OD,w)$
}

\Fn{$\replaceEdge(\OD, v, \ell, w)$}{
    $E(\OD)\gets E(\OD)\setminus\{v\lto{\ell}\ell(v)\}$\;
    $E(\OD)\gets E(\OD)\cup\{v\lto{\ell} w\}$\;
    \Return $\OD$
}

% \Fn{$\DataNode(\OD, d, v_\true)$}{
%     $(\OD,v)\gets \newNode(\OD,\DATA)$\;
%     $\data(v)\gets d$\;
%     $E(\OD)\gets E(\OD)\cup\{v\lto{\true}v_\true\}$\;
%     \Return $(\OD,v)$
% }

% \Fn{$\SourceNode(\OD, v_\true)$}{
%     $(\OD,v)\gets \newNode(\OD,\SOURCE)$\;
%     $\proc(v)\gets \top$\;
%     $E(\OD)\gets E(\OD)\cup\{v\lto{\true}v_\true\}$\;
%     \Return $(\OD,v)$
% }
\end{minipage}\begin{minipage}{.52\linewidth}
% \Fn{$empty()$}{
%     $\OD\gets\text{fresh ordering diagram}$\;
%     $V(\OD)\gets\emptyset;\ E(\OD)\gets\emptyset$\;
%     $(\OD,v)\gets\newNode(\OD,\SINK)$\;
%     $(\OD,u)\gets\SourceNode(\OD,v)$\;
%     $\src(\OD)\gets u;\ \snk(\OD)\gets v$\;
%     \Return $\OD$
% }

% \Fn{$insert(\OD, C, d)$}{
%     /* TODO */\;
%     \Return $\OD$
% }

\Fn{$\replaceEdges(\OD, v, v_\gt, v_\eq, v_\nge)$}{
    $\OD\gets \tsf{replaceEdge}(\OD, v, \gt, v_\gt)$\;
    $\OD\gets \tsf{replaceEdge}(\OD, v, \eq, v_\eq)$\;
    $\OD\gets \tsf{replaceEdge}(\OD, v, \nge, v_\nge)$\;
    \Return $\OD$
}

\Fn{$\newNode(\OD, l)$}{
    $v\gets\text{fresh node};\ \lbl(v)\gets l$\;
    $V(\OD)\gets V(\OD)\cup \{v\}$\;
    \Return $(\OD,v)$
}

\Fn{$\TermNode(\OD, s, t, w_1, w_2, w_3)$}{
    $(\OD,v)\gets \newNode(\OD,\TERM)$\;
    $\lhsT(v)\gets s;\ \rhsT(v)\gets t$\;
    $E(\OD)\gets E(\OD)\cup\{v\lto{\gt}w_1\}$\;
    $E(\OD)\gets E(\OD)\cup\{v\lto{\eq}w_2\}$\;
    $E(\OD)\gets E(\OD)\cup\{v\lto{\nge}w_3\}$\;
    \Return $(\OD,v)$
}

\end{minipage}
\end{algorithm}
%

\begin{algorithm}
\caption{Node inference algorithm}
\Fn{$\inferPath(v)$}{
\Postcond{$\ell$}
    \uIf{$\lbl(v)=\TERM$}{
        $s\gets\lhsT(v);\ t\gets\rhsT(v)$\;
        $\ell\gets\compT(s,t)$\;
        \If{$\ell\neq\true$}{
            \Return $\ell$
        }
        $C'\gets \tsf{transitive\_closure}(C)$\;
        \uIf{$s\succ t\in C'$}{
            \Return $\gt$
        }
        \uElseIf{$s=t\in C'$}{
            \Return $\eq$
        }
        \uElseIf{$s\nsucceq t\in C'$}{
            \Return $\nge$
        }
    }
    \uElseIf{$\lbl(v)=\POLY$}{
        TODO
    }
}
\end{algorithm}

\section{Further improvements}

\begin{itemize}
\item Linearizing terms before inserting them into the index and adding equality constraints instead could be worth investigating.
\item Use per-object arena allocators.
\item Ordering checks on applied terms, i.e. on terms that consist of a term and a substitution to be applied.
\item Fourier-Motzkin elimination or something similar could be used to eliminate variables from polynomials
\item Removal is not described or implemented yet
\item Formalizing it in Dafny/Lean/etc.
\end{itemize}

\subsection*{Demodulation redundancy check}

In forward demodulation, we consider sets of equations $s\eqs t_1$, $s\eqs t_2$, $\ldots$ under a substitution $\theta$.

If $s\theta \succ t_1\theta$ but we fail with the first equation, it is because the additional check in demodulation failed. In this case, we could also check $t_1\theta\nsucceq t_2\theta$, which is needed to check the second equation, and so on.



\begin{figure}[t]
\begin{minipage}{.1\linewidth}
\centering
\begin{tikzpicture}
\node[sourcenode] (source) at (0,1) {};
\node[sinknode] (sink) at (0,0) {};
\altbranch{source}{sink};

\end{tikzpicture}
\end{minipage}\begin{minipage}{.24\linewidth}
\centering
\begin{tikzpicture}
\node[sourcenode] (source) at (0,.7) {};
\node[termnode=left:1] (c1) at (0,0) {$s\comp t$};
\node[datanode=above left:2] (s1) at (0,-1.6) {$s\eqs t$};
\node[sinknode] (sink) at (1,-0.8) {};

\altbranch{source}{c1};

\gtbranch[]{c1}{s1};
\eqbranch[bend right]{c1}{sink};
\incbranch[bend left]{c1}{sink};
\altbranch[]{s1}{sink};

\end{tikzpicture}
\end{minipage}\begin{minipage}{.36\linewidth}
\centering
\begin{tikzpicture}
\node[sourcenode] (source) at (0,.7) {};
\node[termnode=left:1] (c1) at (0,0) {$s\comp t$};
\node[datanode=above left:2] (s1) at (0,-1.6) {$s\eqs t$};
\node[termnode=above:3] (c2) at (1.5,0) {$s\comp u$};
\node[datanode=right:4] (s2) at (1.5,-1.6) {$s\eqs u$};
\node[sinknode] (sink) at (2.5,-0.8) {};

\altbranch{source}{c1};

\gtbranch[]{c1}{s1};
\eqbranch[bend right]{c1}{c2};
\incbranch[bend left]{c1}{c2};

\gtbranch[]{c2}{s2};
\eqbranch[bend right]{c2}{sink};
\incbranch[bend left]{c2}{sink};

\altbranch[]{s1}{c2};
\altbranch[]{s2}{sink};

\end{tikzpicture}

\end{minipage}\begin{minipage}{.3\linewidth}
\centering
\begin{tikzpicture}
\node[sourcenode,draw=none] (source) at (0,.7) {};
\node[termnode=left:1] (c1) at (0,0) {$s\comp t$};
\node[datanode=above left:2] (s1) at (0,-1.6) {$s\eqs t$};
\node[termnode=above:3] (c2) at (1.5,0) {$s\comp u$};
\node[datanode=above right:4] (s2) at (1.5,-1.6) {$s\eqs u$};

\altbranch{source}{c1};

\gtbranch[]{c1}{s1};
\eqbranch[bend right]{c1}{c2};
\incbranch[bend left]{c1}{c2};

\gtbranch[]{c2}{s2};

\altbranch[]{s1}{c2};

\end{tikzpicture}
\end{minipage}

\smallskip

\begin{minipage}{.1\linewidth}
\centering
(a)
\end{minipage}\begin{minipage}{.24\linewidth}
\centering
(b)
\end{minipage}\begin{minipage}{.36\linewidth}
\centering
(c)
\end{minipage}\begin{minipage}{.3\linewidth}
\centering
(d)
\end{minipage}
\caption{Term ordering diagrams over the set of clauses. (a) shows an empty TOD, representing the empty set of indexed pairs, (b) shows a TOD representing an indexed pair $((s\eqs t),\{(s,t)\})$
% ``if $s\theta\succ t\theta$, then $s\eqs t$ for any substitution $\theta$'',
(c) shows a TOD representing two indexed pairs $((s\eqs t),\{(s,t)\})$ and $((s\eqs u),\{(s,u)\})$,
% ``if $s\theta\succ t\theta$, then $s\eqs t$, otherwise if $s\theta\succ u\theta$, then $s\eqs u$ for any substitution $\theta$'',
and (d) shows the same TOD as in (c) with implicit source and sink nodes.}
\label{fig:tod-example}
\end{figure}
%
We illustrate some TODs in the next example. 
%
\begin{example}

Three TODs are displayed in Figure~\ref{fig:tod-example}(a)--(c). Empty circles denote \SOURCE{} nodes, circles filled with black denote \SINK{} nodes, rectangles denote \TERM{} nodes, ellipses denote \POLY{} nodes and diamonds denote \DATA{} nodes. The \terms{} of a \TERM{} node and the \polys{} of a \POLY{} node are shown inside the node separated with a question mark, while the \data{} of a \DATA{} node is simply shown inside the node. A processed node is denoted with bold border. To avoid visual clutter due to edge labels, we present edges labeled \gt{}, \eq{}, \nge{} and \true{} with double lines, dashed lines, zigzag lines and normal lines, respectively.

The smallest possible TOD is shown in Figure~\ref{fig:tod-example}(a), consisting of a \SOURCE{} and \SINK{} node, connected by a \true{} edge. The TOD $\OD$ in Figure~\ref{fig:tod-example}(b) contains additionally one \TERM{} node corresponding to comparing $s$ and $t$ from our motivating example (node 1), and a \DATA{} node containing the unit equation $s\eqs t$ (node 2).
% Note that node 1 has three outgoing edges: its \gt{} edge is connected to node 2, while its \eq{} and \nge{} edges are connected to the sink. The single outgoing edge of node 2 is connected to the sink.
The TOD $\ODprime$ in Figure~\ref{fig:tod-example}(c) contains two more nodes corresponding to comparing $s$ and $u$ (node 3) and storing the unit equation $s\eqs u$ (node 4).

We usually omit displaying source and sink nodes. Figure~\ref{fig:tod-example}(d) shows $\ODprime$ with hidden source and sink nodes. Note that the outgoing edge of $\src(\ODprime)$ is still shown to indicate node 1 as the ``entry point'' of the TOD.\qed
\end{example}
%
We now define the semantics of TODs.
%
\begin{Definition}[TOD semantics]
Let $\OD$ be a TOD and $\theta$ a substitution and let $v$ be a node in $V(\OD)$. We define a function $f_v$ from substitutions to $E(\OD)$.
\begin{enumerate}[label=(\arabic*),itemsep=1pt,parsep=1pt]
\item If $v$ is a \SOURCE{} or \DATA{} node, $f_v(
\theta)=v\lto{\true{}}w$.
\item If $v$ is a \TERM{} node, let $(s,t)=\terms(v)$.
$$f_v(\theta)\defeq\begin{cases}
v\lto{\gt}w &\text{if }s\theta\succ t\theta,\\
v\lto{\eq}w &\text{if }s\theta=t\theta,\\
v\lto{\nge}w &\text{otherwise.}
\end{cases}$$
\item If $v$ is a \POLY{} node, let $(p,q)=\polys(v)$.
$$f_v(\theta)\defeq\begin{cases}
v\lto{\gt}w &\text{if }p\theta> q\theta,\\
v\lto{\eq}w &\text{if }p\theta\not>q\theta\text{ and }p\theta\gtrsim q\theta,\\
v\lto{\nge}w &\text{otherwise.}
\end{cases}$$
\end{enumerate}
We also define a function $\phi_v$ from substitutions to $\mathcal{D}$.
%
\begin{equation*}
\phi_v(\theta)\defeq\begin{cases}
\emptyset&\text{if }v\text{ is \SINK{}},\\
\{\data(v)\}\cup \phi_{w}(\theta)&\text{if }v\text{ is \DATA{}, where }f_v(\theta)=v\lto{\ell}w,\\
\phi_{w}(\theta)&\text{otherwise, where }f_v(\theta)=v\lto{\ell}w.
\end{cases}
\end{equation*}
\qed
\end{Definition}


%
Some remarks are in order. The source and sink nodes of a well-formed TOD make the presentation more clear, but the sink is also used to achieve $\mathcal{O}(1)$ insertion. We use three outgoing edges in a \TERM{} node corresponding to comparison results $\succ$ (\gt{}), $=$ (\eq{}) and $\nsucceq$ (\nge{}) due to the fact that (1) both KBO and LPO definitions use $=$, hence we have to distinguish it from $\succ$, and (2) distinguishing between $\prec$ and $\bowtie$ (incomparability) is usually not needed and experiments suggest that it comes with an undesirable overhead. This choice has some consequences that we will come back to in Section~\ref{sec:path-inference}. The same considerations apply to the outgoing edges of \POLY{} nodes. The sub-requirement in~\ref{prop:well-formed1} that the processed subgraph must be a tree will permit us some further optimizations in addition to simplifying nodes with the definition of the ordering. We come back to this in Section~\ref{sec:path-inference}.

Next, we define a sequence of algorithms that manipulate TODs. To avoid visual clutter, we assume that all algorithms are implicitly given a fixed simplification ordering argument $\succ$. To prove correctness of our algorithms, we will need to compare TODs. First, we define the following helper functions.
%
\begin{align*}
\compT(s,t)&\defeq\begin{cases}
\gt &\text{if }s\succ t,\\
\eq &\text{if }s=t,\\
\nge &\text{otherwise.}
\end{cases}&
\compP(p,q)&\defeq\begin{cases}
\gt &\text{if }p>q,\\
\eq &\text{if }p\not>q\text{ and }p\gtrsim q,\\
\nge &\text{otherwise.}
\end{cases}
\end{align*}
%
\begin{equation*}
\nextF(v,\sigma)\defeq\begin{cases}
\compT(\lhsT(v)\sigma,\rhsT(v)\sigma) &\text{if }\lbl(v)=\TERM,\\
\compP(\sigma_\sigma(\lhsP(v)),\sigma_\sigma(\rhsP(v))) &\text{if }\lbl(v)=\POLY,\\
\true &\text{otherwise.}
\end{cases}
\end{equation*}
%
$\compT$ and $\compP$ compare terms and polynomials, respectively, while $\nextF$ behaves as a ``successor'' function for a TOD node $v$ w.r.t. a substitution $\sigma$. Given a substitution $\sigma$, the following function computes the content of a TOD subdiagram stemming at a node $v$ algebraically.
%
\begin{equation*}
\phi(v,\sigma)\defeq\begin{cases}
\langle\rangle&\text{if }\lbl(v)=\SINK,\\
\langle\data(v)\rangle\cons \phi(\ell(v),\sigma)&\text{if }\lbl(v)=\DATA,\\
\phi(\ell(v),\sigma)&\text{otherwise,}
\end{cases}
\end{equation*}
where $\ell=\nextF(v,\sigma)$. Finally, we use the following definition to compare TODs.
%
\begin{Definition}[TOD Equivalence]
Let $\OD$ and $\ODprime$ be TODs. We say that $\OD$ and $\ODprime$ are \emph{equivalent}, denoted by $\OD\sim\ODprime$, if for each substitution $\sigma$, we have $\phi(\src(\OD),\sigma)=\phi(\src(\ODprime),\sigma)$.\qed
\end{Definition}
%
The following lemma states that there is a unique path in a well-formed TOD from the source to the sink given a substitution.
%
\begin{lemma}[TOD Trace Uniqueness]
\label{lem:trace-uniqueness}
Let $\OD$ be a well-formed TOD and $\sigma$ a substitution. There is exactly one path $\src(\OD)=u_1\lto{\ell_1}u_2\lto{\ell_2}\ldots \lto{\ell_{n-1}}u_n\lto{\ell_n}\snk(\OD)$ in $\OD$ s.t. $\ell_i=\nextF(u_i,\sigma)$ for all $1\le i \le n$.
\end{lemma}
\begin{proof}
It follows from the definitions of well-formedness and \nextF.\qed
\end{proof}
%
We call the path in Lemma~\ref{lem:trace-uniqueness} for a given TOD $\OD$ and substitution $\sigma$ the \emph{trace in $\OD$ w.r.t. $\sigma$} and denote it with $\trace(\OD,\sigma)$.

Finally, for termination of our algorithms, we define an ordering $\gtrdot$ between well-formed TODs.
\begin{Definition}[Ordering $\gtrdot$]
Let $\OD$ be a well-formed TOD. We define the multiset of paths $M_P$ for each $v\in V(\OD)$ as:
%
$$M_P(v)\defeq\begin{Bmatrix}\{v\}\uplus m\mid m\in \biguplus_{v\to w\in E(\OD)} M_P(w)\end{Bmatrix}$$
%
Let $u$ and $v$ be two nodes. We define a total relation $>_l$ between node labels as $\TERM{}>_l\POLY{}>_l\DATA{}>_l\SOURCE{}>_l\SINK$. Additionally, let $\|\cdot\|$ denote the size of an expression. We also define $\proc(v)>\neg\proc(v)$. We write $u>v$ if $(\lbl(u),\|\lhsT(u)\|+\|\rhsT(u)\|,\proc(u))>_{lex}(\lbl(v),\|\lhsT(v)\|+\|\rhsT(v)\|,\proc(v))$\todo{Robin: This is notation heavy and difficult to follow. Is there a way to make it lighter?}. Let $\OD$ and $\ODprime$ be TODs. We write $\OD\gtrdot\ODprime$ if $M_P(\src(\OD))(>_{mul})_{mul}M_P(\src(\ODprime))$.\qed\todo{Define these precisely.}
\end{Definition}
%
\begin{restatable}[Well-foundedness of $\gtrdot$]{lemma}{wellfoundedness}
The relation $\gtrdot$ on TODs is well-founded.
\end{restatable}
\begin{proof}
It is well-known that the lexicographic product of well-founded orders is well-founded, and that the multiset extension of a well-founded order over finite multisets is well-founded. A well-formed TOD is a finitely-branching DAG, so the multisets defined by $M_P$ are finite. $>_l$ is obviously well-founded, so as comparing expression sizes and the relation $\proc(v)>\neg\proc(v)$.\qed
\end{proof}

%
% \subsection{Creation and Insertion}
% %
% We make use of the functions shown in Algorithm~\ref{alg:miscellaneous} to create new nodes and TODs. For node removal, we assume that whenever a node other than the root $r$ becomes unreachable, it is removed from the set of vertices $V$. This can be done similarly in practice by e.g. reference counting.
% %
% We create initial TODs for a single ordering constraint associated with some data. For example, Figure~\ref{fig:tod-example}(a)--(b) shows two TODs for the two demodulators $s\eqs t$ and $s\eqs u$ and their ordering constraints.
%


\begin{minipage}{.4\linewidth}

\begin{center}
\begin{tikzpicture}[canvassed]
\node[] (source) at (0,.7) {};
\node[termnode] (c1) at (0,0) {$l\comp r_1$};
\node[datanode] (s1) at (0,-2) {$l\eqs r_2$};
\node[termnode] (c2) at (2.5,0) {$l\comp r_1$};
\node[datanode] (s2) at (2.5,-2) {$l\eqs r_2$};

\altbranch{source}{c1};
\draw[->] (c1) -- node[midway,gtedgenode]{} (s1);
\draw[->] (c1) edge[bend left=15] node[midway,eqedgenode]{} (c2);
\draw[->] (c1) edge[bend right=15] node[midway,ngeqedgenode]{} (c2);
\draw[->] (s1) -- (c2);
\draw[->] (c2) -- node[midway,gtedgenode]{} (s2);

\end{tikzpicture}
\end{center}

\end{minipage}\begin{minipage}{.6\linewidth}

\begin{center}
\begin{tikzpicture}[canvassed]
\node[] (source) at (0,.7) {};
\node[polynode] (c1) at (0,0) {$0\pos 0$};
\node[termnode] (c2) at (0,-2) {$x\comp y$};
\node[termnode] (c3) at (0,-4) {$y\comp x$};
\node[datanode] (s1) at (0,-6) {$l\eqs r_1$};
\node[termnode] (c4) at (3,-2) {$l\comp r_2$};
\node[datanode] (s2) at (3,-4) {$l\eqs r_2$};

\altbranch{source}{c1};
\draw[->] (c1) -- (-1,-2) edge[bend right] node[pos=0,gtedgenode]{} (s1);
\draw[->] (c1) -- node[geqedgenode]{} (c2);
\draw[->] (c1) -- node[ngeqedgenode]{} (c4);

\draw[->] (c2) -- (-.9,-4) -- node[pos=0,gtedgenode]{} (s1);
\draw[->] (c2) -- node[eqedgenode]{} (c3);
\draw[->] (c2) -- node[ngeqedgenode]{} (c4);

\draw[->] (c3) -- node[gtedgenode]{} (s1);
\draw[->] (c3) edge[bend left=10] node[eqedgenode]{} (c4);
\draw[->] (c3) edge[bend right=10] node[ngeqedgenode]{} (c4);

\draw[->] (s1) -- (c4);

\draw[->] (c4) -- node[gtedgenode]{} (s2);

\end{tikzpicture}
\end{center}

\end{minipage}\\


\begin{minipage}{.5\linewidth}

\begin{center}
\begin{tikzpicture}[canvassed]
\node[] (source) at (0,.7) {};
\node[termnode] (c1) at (0,0) {$x\comp y$};
\node[termnode] (c2) at (0,-2) {$y\comp x$};
\node[datanode] (s1) at (0,-4) {$l\eqs r_1$};
\node[termnode] (c3) at (3,0) {$l\comp r_2$};
\node[datanode] (s2) at (3,-2) {$l\eqs r_2$};

\altbranch{source}{c1};

\draw[->] (c1) -- (-.9,-2) -- node[pos=0,gtedgenode]{} (s1);
\draw[->] (c1) -- node[eqedgenode]{} (c2);
\draw[->] (c1) -- node[ngeqedgenode]{} (c3);

\draw[->] (c2) -- node[gtedgenode]{} (s1);
\draw[->] (c2) edge[bend left=10] node[eqedgenode]{} (c3);
\draw[->] (c2) edge[bend right=10] node[ngeqedgenode]{} (c3);

\draw[->] (s1) -- (c3);

\draw[->] (c3) -- node[gtedgenode]{} (s2);

\end{tikzpicture}
\end{center}

\end{minipage}\begin{minipage}{.5\linewidth}

\end{minipage}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\linewidth]{plots/discount-kbo.png}
    \includegraphics[width=0.49\linewidth]{plots/discount-lpo.png}
    \includegraphics[width=0.49\linewidth]{plots/otter-kbo.png}
    \includegraphics[width=0.49\linewidth]{plots/otter-lpo.png}
    % \resizebox{0.49\textwidth}{!}{\input{plots/discount-kbo.pgf}}
    % \resizebox{0.49\textwidth}{!}{\input{plots/discount-lpo.pgf}}
    % \resizebox{0.49\textwidth}{!}{\input{plots/otter-kbo.pgf}}
    % \resizebox{0.49\textwidth}{!}{\input{plots/otter-lpo.pgf}}
    \caption{Relative speedup by number of instructions plotted on the y-axis of configuration on x-axis compared to {\tt -fdtod off}. Each data point is a benchmark solved by both {\tt -fdtod off} and the respective configuration on the x-axis.}
    \label{fig:evaluation}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\linewidth]{plots/discount-kbo_cactus.png}
    \includegraphics[width=0.49\linewidth]{plots/discount-lpo_cactus.png}
    \includegraphics[width=0.49\linewidth]{plots/otter-kbo_cactus.png}
    \includegraphics[width=0.49\linewidth]{plots/otter-lpo_cactus.png}
    \caption{Cactus plot, x-axis shows millions of executed instructions, y-axis shows number of benchmarks solved. TODO. "Solved" is misleading here since time limit was used and not instruction limit.}
    \label{fig:evaluation2}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\linewidth]{plots/discount-kbo_memory.png}
    \includegraphics[width=0.49\linewidth]{plots/discount-lpo_memory.png}
    \includegraphics[width=0.49\linewidth]{plots/otter-kbo_memory.png}
    \includegraphics[width=0.49\linewidth]{plots/otter-lpo_memory.png}
    \caption{TODO. Memory usage shown similarly as in Figure~\ref{fig:evaluation}. Not sure if useful.}
    \label{fig:evaluation3}
\end{figure}

Our algorithm works as follows. Let $\OD$ be a TOD and $u\lto{\ell}v\in E(\OD)$ s.t. $u$ is processed. Since $u$ is part of $\proc(\OD)$, there is a unique path leading to this node which does not change in further steps of our algorithm. We overapproximate the set of substitutions $\theta$ which lead to $u$ in our traversal algorithm by collecting a conjunction of constraints. For example, an edge $u'\lto{\ell'}v'$ on this path where $\lbl(u')=\TERM{}$, $\lhsT(u')=s$, $\rhsT(u')=t$ and $\ell'=\gt$ means that any substitution leading to $v'$ must satisfy $s\theta\succ t\theta$. We turn this into a \emph{term constraint} $s>t$. Similarly, we get term constraints of the form $s=t$ if $\ell'=\eq$, and $s\ngeq t$ if $\ell'=\nge$. For \POLY{} nodes we get \emph{linear constraints} of the form $p>q$, $p\geq q$ and $p\ngeq q$.

Our algorithm consists of two parts. We use term constraints to infer the outgoing edges of \TERM{} nodes using a transitive closure algorithm, and linear constraints are used for inferring outgoing edges of \POLY{} nodes. In some cases, it is possible to convert term constraints into linear constraints and vice versa. For example, a term constraint $s>t$ or $s=t$ is turned into $|s|\geq|t|$, while a linear constraint such as $x>1+y$ can be turned into any term constraint $s>t$ where $s$ and $t$ are arbitrary terms that satisfy the above equation by the definition of KBO.

For inferring the outgoing edge of $v$ if it is a \TERM{} node, we use a transitive closure algorithm over term constraints. Since we also have negative term constraints, in addition to usual transitivity rules, we also use the following three rules:
%
\begin{align*}
s \leq t \land t \ngeq u \to s \ngeq u\\
s \ngeq t \land t \leq u \to s \ngeq u\\
s \nleq t \land s \ngeq t \to s \bowtie t
\end{align*}
%
We infer outgoing edges of \POLY{} nodes by using Fourier-Motzkin elimination.
